Real-time Prediction of COVID-19 related Mortality using Electronic Health Records

Coronavirus Disease 2019 (COVID-19) is an emerging respiratory disease caused by the severe acute respiratory syndrome coronavirus 2 (SARS-CoV-2) with rapid human-to-human transmission and a high case fatality rate particularly in older patients. Due to the exponential growth of infections, many healthcare systems across the world are under pressure to care for increasing amounts of at-risk patients. Given the high number of infected patients, identifying patients with the highest mortality risk early is critical to enable effective intervention and optimal prioritisation of care. Here, we present the COVID-19 Early Warning System (CovEWS), a clinical risk scoring system for assessing COVID-19 related mortality risk. CovEWS provides continuous real-time risk scores for individual patients with clinically meaningful predictive performance up to 192 hours (8 days) in advance, and is automatically derived from patients' electronic health records (EHRs) using machine learning. We trained and evaluated CovEWS using de-identified data from a cohort of 66430 COVID-19 positive patients seen at over 69 healthcare institutions in the United States (US), Australia, Malaysia and India amounting to an aggregated total of over 2863 years of patient observation time. On an external test cohort of 5005 patients, CovEWS predicts COVID-19 related mortality from $78.8\%$ ($95\%$ confidence interval [CI]: $76.0$, $84.7\%$) to $69.4\%$ ($95\%$ CI: $57.6, 75.2\%$) specificity at a sensitivity greater than $95\%$ between respectively 1 and 192 hours prior to observed mortality events - significantly outperforming existing generic and COVID-19 specific clinical risk scores. CovEWS could enable clinicians to intervene at an earlier stage, and may therefore help in preventing or mitigating COVID-19 related mortality.

==> survival_analysis.tex <==
We train, test, and validate our method for an early warning score for mortality prediction on routinely collected data from clinical measurements, lab tests, and information about pre-existing conditions of \numprint{44842} patients from Optum's database. To show the potential applicability of the proposed CovScore in clinical practice, we additionally validate the approach on a complete hold-out dataset of a different research database. We report the survival probability that intuitively shows how urgent the condition of a patient is at a certain time. It is defined as the cumulative hazard up to a target time where the hazard is the conventional hazard function in a Cox model~\cite{cox1972regression}.

\paragraph{Survival analysis:} To verify if the estimated risk score defined in  \eqref{eq:cox_hazard_nonlinear_body} is predictive of the actual survival, patients are categorized into five strata according to their estimated risk score at time $t$. The lowest $60\%$ is assigned to stratum 0 and the top $10\%$ of the risk scores are assigned to stratum $4$. The intermediate risk scores are divided into $3$ strata as shown in~\Cref{fig:survival_curves_optum}. While other splits are possible, five strata are chosen for visualization reasons. Notice that these curves are different from traditional survival functions which are usually plotted for a fixed population. Here, the strata do not correspond to a pre-specified fixed set of patients. They correspond to specified percentiles of the risk score. Hence, a patient may join or leave a stratum when its covariates change. The instantaneous value of the covariates of each patient determines which risk group it belongs to at time $t$. A patient may be at a high-risk group at time $t_0$ but change into a lower risk group when its covariates change due to treatment or self-healing at time $t_1$. Therefore, in time-varying setting, the survival plots predict the survival probability of a risk group rather than a certain patient. To predicted risk scores need to be calibrated to be comparable across populations and models. The calibration plots for the trained model for both Optum's and TriNetX data can be found in~\Cref{fig:calibration_curves} in the supplement. Each point of the calibration curve maps the output risk score of the model to the actual risk. A perfectly calibrated model has an exact linear curve with a slope of $45^\circ$. 

To verify the capability of the learned hazard function in stratification, the Kaplan-Meier curves for each stratum are plotted in~\Cref{fig:survival_curves_optum}. Recall that Kaplan-Meier estimators depend only on the number of deaths and the total number of people at risk at each time. In other words, these estimators are not a function of the covariates of the patient and only look at the outcome -- survival or death. It is seen in~\Cref{fig:survival_curves_optum} that patients who are categorized in strata with higher risks have steeper survival curves. This implies that the trained hazard model~\labelcref{eq:survival_function_main} is actually predictive of the survival chance of the patient at each time.

The number of people at risk and the cumulative number of deaths from each stratum are shown in~\Cref{fig:survival_curves_optum} as well. The last stratum (pale red) has the least number of people at risk with a higher number of cumulative deaths, which thus identifies this stratum as the group of patients requiring interventions with the highest priority. The order of the risk scores assigned to other strata is aligned with the observed mortality of each group. This alignment suggests that the trained model captures the risk that a patient is facing at each point in time based on its covariates at that point.

Similar survival analysis is performed for the external hold-out dataset from TriNetX. In~\Cref{fig:survival_curves_trinetx} shows that the trained and validated model on the Optum's data likewise works well on the TriNetX's data by stratification of the risk group based on their instantaneous covariates. This empirical observation suggests that the model trained on routinely collected EHRs, can potentially generalize to other sources of data collected with different protocols or from different locations.


\paragraph{Prediction Time Frame} To compare the performance of our method against already peer-reviewed mortality prediction baselines for COVID-19 e.g. \cite{yan2020interpretable}, we have plotted the specificity of models with a fixed sensitivity of $95\%$ for a different number of hours until the time of mortality in~\Cref{fig:baselines}. The validation is performed on both the hold-out test subset of Optum's data (left) and the external hold-out data from TriNetX (right). As expected, all methods give more accurate predictions in shorter time-frames. At each time-frame, our method outperforms other baselines with a significant margin. Moreover, it can be seen that even though the performance of all methods gets worse on TriNetX's data, our method still outperforms other methods indicating the potential generalizability of our method to various data collectors and various locations.



% \ar{merged in the previous paragraph: Comparison to other baselines: Comparisons with  already peer-reviewed mortality prediction models for COVID-19 patients \cite{yan2020interpretable} can be found in Figure \ref{fig:baselines} as well in the supplement \ref{sec:supp_comparisons}. Overall we observe that our method significantly outperforms the existing baselines in terms of specificity across several different prediction timeframes. Evidently, these predictions are more accurate closer to the time of the event and tend to drop slightly as the number of hours before the event increases. This difference in performance is sustained across the external validation set. }


